Modeling Supervisor Safe Sets for Improving Collaboration in Human-Robot Teams

When a human supervisor collaborates with a team of robots, their attention is divided and cognitive resources are at a premium. We aim to optimize the distribution of these resources and the flow of attention. To this end, we propose the model of an idealized supervisor to describe human behavior. Such a supervisor employs a potentially inaccurate internal model of the the robots' dynamics to judge safety. We represent these safety judgements by constructing a safe set from this internal model using reachability theory. When a robot leaves this safe set, the idealized supervisor will intervene to assist, regardless of whether or not the robot remains objectively safe. False positives, where a human supervisor incorrectly judges a robot to be in danger, needlessly consume supervisor attention. In this work, we propose a method that decreases false positives by learning the supervisor's safe set and using that information to govern robot behavior. We prove that robots behaving according to our approach will reduce the occurrence of false positives for our idealized supervisor model. Furthermore, we empirically validate our approach with a user study that demonstrates a significant ($p = 0.0328$) reduction in false positives for our method compared to a baseline safety controller.

==> background.tex <==
\subsection{Reachability and Safe Sets}
\label{sec:reachability}
Safe sets are predicated upon the Formal Methods notion of ``Viability''.
A set of states is ``viable'' if for every state in the set there exists a dynamic trajectory that stays within the set for all time.
Reachability analysis calculates the largest viable set that doesn't include any undesirable state configurations (e.g. collisions with obstacles, power overloads, etc).
Since the set is viable, it is possible to guarantee that the dynamic system will always stay within the set and therefore stay safely away from the undesirable states.
For this reason, viability kernels are often referred to as ``safe sets''.
Reachability can be used for robust path planning in dynamically changing environments \cite{fisac2015reach} or working around multiple dynamic agents \cite{chen2015safe}, and recent results have leveraged the technique to bound tracking error in order to generate dynamically feasible paths using simple planning algorithms \cite{FaSTrack}.

Hoffman et al. used the safety guarantees of reachability analysis to engineer a multi-drone team that could automatically avoid collisions \cite{hoffmannCollisionAvoidance}.
Similarly, Gillula could guarantee safety for learning algorithms by constraining their explorations to stay within the safe set \cite{gillulaMinimallyInvasive}.
Extending this, Akametalu and Tomlin \cite{KeneReachLearning} were able to guarantee safety while simultaneously learning and expanding the safe set.
All of these controllers supervise otherwise un-guaranteed systems and intervene to maintain safety whenever the system threatens to leave the viable safe set.
In this paper, we explore how this intervention behavior is similar to human supervision, and apply this to representing human safety concerns as safe sets in the state space.

%Reachability can be used for robust path planning in dynamically changing environments \cite{fisac2015reach}, or working around multiple dynamic agents \cite{chen2015safe}, and recent results have leveraged the technique to bound tracking error to render dynamically feasible paths using simple planning algorithms \cite{FaSTrack}.

\subsection{Cognitive Dynamical Models}
Cognitive science gives psychology new ways of modeling human reasoning which in turn gives AI new ways to work with human agents.
Inspired by linguistic pragmatics, Dragan et al. modeled humans observing robot behavior as Bayesian inference engines, which in turn allowed them to optimize trajectories for communicating intent \cite{dragan2013legibility}.
Work in neuromechanical motor control asserts that human action mastery involves building a dynamical model of the human body \cite{shadmehr1994adaptive}.
Robinson et. al posited that this dynamics learning extends not just to direct control of the body but to systems less directly controlled by the human such as Human-Cyberphysical systems \cite{robinsonDynamicInverseModels}.
Similarly, the ``Noisy Newton'' hypothesis models human general scene-understanding as mentally executing noisy physics simulators, and recent studies are supporting this model \cite{HamrickSim} \cite{StochasticMentalSim}.

